Efficient deep data assimilation with sparse observations and time-varying sensors

Variational Data Assimilation (DA) has been broadly used in engineering problems for field reconstruction and prediction by performing a weighted combination of multiple sources of noisy data. In recent years, the integration of deep learning (DL) techniques in DA has shown promise in improving the efficiency and accuracy in high-dimensional dynamical systems. Nevertheless, existing deep DA approaches face difficulties in dealing with unstructured observation data, especially when the placement and number of sensors are dynamic over time. We introduce a novel variational DA scheme, named Voronoi-tessellation Inverse operator for VariatIonal Data assimilation (VIVID), that incorporates a DL inverse operator into the assimilation objective function. By leveraging the capabilities of the Voronoi-tessellation and convolutional neural networks, VIVID is adept at handling sparse, unstructured, and time-varying sensor data. Furthermore, the incorporation of the DL inverse operator establishes a direct link between observation and state space, leading to a reduction in the number of minimization steps required for DA. Additionally, VIVID can be seamlessly integrated with Proper Orthogonal Decomposition (POD) to develop an end-to-end reduced-order DA scheme, which can further expedite field reconstruction. Numerical experiments in a fluid dynamics system demonstrate that VIVID can significantly outperform existing DA and DL algorithms. The robustness of VIVID is also accessed through the application of various levels of prior error, the utilization of varying numbers of sensors, and the misspecification of error covariance in DA.

==> name.tex <==
    \bB_t\left(\frac{\bB_t^2 \bH^2_t}{\bB_t \bH^2_t \bP_t+\bB_t \bR_t+\bP_t \bR_t}-\frac{\bB_t\left(\bB_t \bH^2_t+r\right)}{\bB_t \bH^2_t \bP_t+\bB_t \bR_t+\bP_t \bR_t}-h\left(-\frac{\bB_t^2 h}{\bB_t \bH^2_t \bP_t+\bB_t \bR_t+\bP_t \bR_t}+\frac{\bB_t h(\bB_t+\bP_t)}{\bB_t \bH^2_t \bP_t+\bB_t \bR_t+\bP_t \bR_t}\right)+1\right)
